Developers Perception of Peer Code Review in Research Software Development

Background: Research software is software developed by and/or used by researchers, across a wide variety of domains, to perform their research. Because of the complexity of research software, developers cannot conduct exhaustive testing. As a result, researchers have lower confidence in the correctness of the output of the software. Peer code review, a standard software engineering practice, has helped address this problem in other types of software. Aims: Peer code review is less prevalent in research software than it is in other types of software. In addition, the literature does not contain any studies about the use of peer code review in research software. Therefore, through analyzing developers perceptions, the goal of this work is to understand the current practice of peer code review in the development of research software, identify challenges and barriers associated with peer code review in research software, and present approaches to improve the peer code review in research software. Method: We conducted interviews and a community survey of research software developers to collect information about their current peer code review practices, difficulties they face, and how they address those difficulties. Results: We received 84 unique responses from the interviews and surveys. The results show that while research software teams review a large amount of their code, they lack formal process, proper organization, and adequate people to perform the reviews. Conclusions: Use of peer code review is promising for improving the quality of research software and thereby improving the trustworthiness of the underlying research results. In addition, by using peer code review, research software developers produce more readable and understandable code, which will be easier to maintain.

==> novelty_statement.tex <==
\textbf{Novelty Statement}
This paper reports on new results that have not appeared in previous publications.
The contents of this paper are novel.

==> sec_research_questions.tex <==

To drive the overall study design, we identified four research questions.
In this section, we introduce each research question by providing a brief motivation for why the question is important and relevant.
We also describe the type of information necessary to answer the question.

\vspace{8pt}
\noindent
\textbf{RQ1: How do research software developers perform peer code review?}

\noindent
While there is extensive research on peer code review in commercial and open source software, there is no empirical research on the use of peer code review in research software.
Therefore, we must first gain a basic understanding of the process research software developers follow when performing peer code review.
To answer this question, we need to gather details about the peer code review process research software developers follow along with their positive and negative experiences.

\vspace{8pt}
\noindent
\textbf{RQ2: What effect does peer code review have on research software?}

\noindent
The goal of this question is to understand whether the benefits of peer code review seen in open source and commercial software (discussed in the previous section) also appear in research software.
To understand the prevalence of these benefits, we need to gather information about how peer code review impacts research software.


\vspace{8pt}
\noindent
\textbf{RQ3: What difficulties do research software developers face with peer code review?}

\noindent
In addition to the benefits of peer code review, the previous section identifies some of the difficulties in performing peer code review.
This research question seeks to understand whether those difficulties also hold for research software.
We need to collect information about the challenges and barriers research software developers face.

\vspace{8pt}
\noindent
\textbf{RQ4: What improvements to the peer code review process do research software developers need?}

\noindent
Similar to the improvements to tooling, processes, and investments commercial and open-source projects have made relative to the peer code review process (as discussed in the previous section), this question seeks to understand changes that could help peer code review for research software.
To answer this question we need to gather information about the gaps in the process and the desired improvements.
